Notes on Applicability of GPT-4 to Document Understanding

We perform a missing, reproducible evaluation of all publicly available GPT-4 family models concerning the Document Understanding field, where it is frequently required to comprehend text spacial arrangement and visual clues in addition to textual semantics. Benchmark results indicate that though it is hard to achieve satisfactory results with text-only models, GPT-4 Vision Turbo performs well when one provides both text recognized by an external OCR engine and document images on the input. Evaluation is followed by analyses that suggest possible contamination of textual GPT-4 models and indicate the significant performance drop for lengthy documents.

==> tldr.tex <==
\begin{figure*}[!ht]
    \awesomebox[tab1]{2pt}{\faInfoCircle}{tab1}{%
        \textbf{TL;DR:} Though it is hard to achieve good results with text-only models, GPT-4 Vision Turbo performs decently with documents represented as a series of $2048$px images. Its performance can be significantly improved if one provides text recognized by an external OCR engine in addition to images, even if the text is of low quality. The performance drops considerably with the length of the document and, in most cases, is below the state-of-the-art Document Understanding solutions.
    }
\end{figure*}
